OmniBoost: Boosting Throughput of Heterogeneous Embedded Devices under Multi-DNN Workload

Modern Deep Neural Networks (DNNs) exhibit profound efficiency and accuracy properties. This has introduced application workloads that comprise of multiple DNN applications, raising new challenges regarding workload distribution. Equipped with a diverse set of accelerators, newer embedded system present architectural heterogeneity, which current run-time controllers are unable to fully utilize. To enable high throughput in multi-DNN workloads, such a controller is ought to explore hundreds of thousands of possible solutions to exploit the underlying heterogeneity. In this paper, we propose OmniBoost, a lightweight and extensible multi-DNN manager for heterogeneous embedded devices. We leverage stochastic space exploration and we combine it with a highly accurate performance estimator to observe a x4.6 average throughput boost compared to other state-of-the-art methods. The evaluation was performed on the HiKey970 development board.

==> pics/loss.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions = {size
    \convertlen{0.48\textwidth}, 3.9cm font ',7'}]

set border
set key right top width 4 spacing 1.4 

set grid

set title 'Throughput estimator training behavior' offset 0, 0.5,0

set ylabel "Loss"
set ylabel offset -1.5,0,0
set ytics 0, 0.05
set yrange [ 0.10 : 0.35 ] noreverse writeback
set datafile missing "NaN"

set xtics nomirror
set xlabel 'Epoch'

set xrange [0:100]
set xtics 10

set style line 1 linecolor rgb '#0060ad' linetype 1 linewidth 3.0 pointtype 2 pointsize 0.0
set style line 2 linecolor rgb '#dd181f' linetype 1 linewidth 3.0 pointtype 3 pointsize 0.0
set style line 3 lc rgb '#0060ad' linetype 1 linewidth 3.0 pointtype 7 pointsize 0.0
set style line 4 lc rgb '#09ad00' linetype 1 linewidth 3.0 pointtype 5 pointsize 0.0
set style line 5 lc rgb '#b72ad4' linetype 1 linewidth 3.0 pointtype 5 pointsize 0.0

set rmargin 0

set arrow from 38, 0.12 to 38, 0.33 nohead lw 3 lt 7 dt 2
set label 1 at 40, 0.25 'Convergence '

plot "./data/loss.dat" using 1:2 with linespoints linestyle 4 title 'Training loss', \
'' using 1:3 with linespoints linestyle 3 title 'Validation loss'


\end{gnuplot}


==> pics/mix3.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions = {size
    \convertlen{0.48\textwidth}, 3.9cm font ',7'}]

set pm3d map
set palette rgb 23,28,3

set key right top horizontal
set key outside

set rmargin 0
set border
set grid
set boxwidth 0.8
set style histogram cluster gap 1
set style fill solid 1.00 
set format y '%1.1f'
set yrange [0 to 2.0]
set ylabel 'Average Normalized throughput'
set ytics 0, 0.5

set style data histograms

plot "data/mix3.dat" using 2:xtic(1) title 'Baseline' lc rgb '#fec44f' ,\
     "" using 3 title 'MOSAIC \cite{han2019mosaic}' lc rgb '#fe9929' , \
     "" using 4 title 'GA \cite{kang2020scheduling}' lc rgb '#d95f0e', \
     "" using 5 title 'OmniBoost' lc rgb '#993404', 

\end{gnuplot}   


==> pics/mix4.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions = {size
    \convertlen{0.48\textwidth}, 3.9cm font ',7'}]

set pm3d map
set palette rgb 23,28,3

set key right top horizontal
set key outside

set rmargin 0
set border
set grid
set boxwidth 0.8
set style histogram cluster gap 1
set style fill solid 1.00 
set format y '%1.1f'
set yrange [0 to 7.5]
set ylabel 'Average Normalized throughput'
set ytics 0, 1.5

set style data histograms

plot "data/mix4.dat" using 2:xtic(1) title 'Baseline' lc rgb '#fec44f' ,\
     "" using 3 title 'MOSAIC \cite{han2019mosaic}' lc rgb '#fe9929' , \
     "" using 4 title 'GA \cite{kang2020scheduling}' lc rgb '#d95f0e', \
     "" using 5 title 'OmniBoost' lc rgb '#993404', 

\end{gnuplot}   


==> pics/mix5.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions = {size
    \convertlen{0.48\textwidth}, 3.9cm font ',7'}]

set pm3d map
set palette rgb 23,28,3

set key right top horizontal
set key outside

set rmargin 0
set border
set grid
set boxwidth 0.8
set style histogram cluster gap 1
set style fill solid 1.00 
set format y '%1.1f'
set yrange [0 to 1.5]
set ylabel 'Average Normalized throughput'
set ytics 0, 0.5

set style data histograms

plot "data/mix5.dat" using 2:xtic(1) title 'Baseline' lc rgb '#fec44f' ,\
     "" using 3 title 'MOSAIC \cite{han2019mosaic}' lc rgb '#fe9929' , \
     "" using 4 title 'GA \cite{kang2020scheduling}' lc rgb '#d95f0e', \
     "" using 5 title 'OmniBoost' lc rgb '#993404', 

\end{gnuplot}   


==> pics/motivation.tex <==
\begin{gnuplot}[terminal=cairolatex, terminaloptions = {size
    \convertlen{0.48\textwidth}, 3.6cm font ',7'}] 

set border
unset key
set grid

set ylabel "Normalized throughput" 
set xlabel "Different set-ups" 

#set ytics format "%1.0f"
set yrange [ 0 : 1.8 ] noreverse nowriteback

set arrow from 0, 1 to 200, 1 nohead lw 3 lt 7 

plot "./data/motivational.dat" using 1:2 with points pointtype 7 pointsize 0.5

\end{gnuplot}

